Reaching diffraction-limited localization with coherent PTAs

Current pulsar timing array (PTA) analyses do not take full advantage of pulsar distance information, thereby missing out on improved angular resolution and on a potential factor-of-two gain in detection sensitivity for individual gravitational-wave (GW) sources. In this work, we investigate the impact of precise pulsar distance measurements on angular resolution as an extension to previous work measuring the angular resolution of a dense, isotropic PTA [Jow et al., 2025]. We present a coherent map-making technique that utilizes precise pulsar distance measurements to reach the diffraction-limited resolution of an individual source: $\delta \theta_{\mathrm{diff}} \sim (1/\mathrm{SNR})(\lambda_{\mathrm{GW}}/r) \approx 2~\mathrm{arcmin}$, where the SNR refers to the detection strength of the source. With this level of angular resolution, identifying an EM counterpart may become feasible, enabling multi-messenger follow-up. We show that for $\rm SNR=10$, which may be the current sensitivity level using a coherent analysis, the diffraction limit is reached with roughly 9 pulsars. Moreover, angular resolution scales sharply with the number of known pulsar distances as $\sim (1/\mathrm{SNR})^{N_{\mathrm{dist}}/2}$. Thus, each additional pulsar with high signal-to-noise timing and precise distance measurement can improve PTA resolution by an order of magnitude. The distance to the best-timed millisecond pulsar (PSR J0437$-$4715) is already constrained to sub-parsec levels. We argue, therefore, that a coherent analysis of PTA data, fully incorporating pulsar distance information, is timely.

==> PRL_Justification.tex <==
% PRL justification statement

% focus on finding EM counter parts
Finding EM counterparts to nanohertz GWs detected by PTAs for standard-siren analyses requires high-precision source localization, which is not achievable without precise constraints on pulsar distances. We show that the maximum, diffraction-limited resolution is achieved with approximately nine sub-parsec distance measurements. Each additional pulsar distance improves angular resolution by approximately an order of magnitude. Precision pulsar distance measurements enable GW phase constraints, potentially doubling the sensitivity to individual sources. There are already sub-parsec distance constraints on the best-timed millisecond pulsar, motivating the urgent need for coherent approaches to PTA analysis such as ours.
